Language and Intelligence, Artificial vs. Natural or What Can and What Cannot AI Do with NL?

In this talk, I argue that there are certain pragmatic features of natural language (that I will call 'productivity' and 'malleability', on top of syntactical generativity and semantical compositionality), which are not only hard, but even impossible to capture in an artificial language used by an AI system, and the reason for this is to be found in certain deep, metaphysical differences between artificial and natural intelligence, accounting for the differences in their respective processes of concept-formation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{H. Bordihn, G. Horv\'ath, G. Vaszil (Eds.): 12th International Workshop on\\Non-Classical Models of Automata and Applications (NCMA 2022)\\
EPTCS 367, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.367.1}{10.4204/EPTCS.367.1}}
\pdfoutput=1

